Optimizing Tensor Programs on Flexible Storage

Tensor programs often need to process large tensors (vectors, matrices, or higher order tensors) that require a specialized storage format for their memory layout. Several such layouts have been proposed in the literature, such as the Coordinate Format, the Compressed Sparse Row format, and many others, that were especially designed to optimally store tensors with specific sparsity properties. However, existing tensor processing systems require specialized extensions in order to take advantage of every new storage format. In this paper we describe a system that allows users to define flexible storage formats in a declarative tensor query language, similar to the language used by the tensor program. The programmer only needs to write storage mappings, which describe, in a declarative way, how the tensors are laid out in main memory. Then, we describe a cost-based optimizer that optimizes the tensor program for the specific memory layout. We demonstrate empirically significant performance improvements compared to state-of-the-art tensor processing systems.

==> abstract.tex <==
\begin{abstract}
OBSOLETE.  EDIT main.tex INSTEAD

  Tensor programs often need to process large tensors (vectors,
  matrices, or higher order tensors) that require a specialized
  storage format for their memory layout.  Several such layouts have
  been proposed in the literature, such as the Coordinate Format, the
  Compressed Sparse Row format, and many others, that were especially
  designed to store optimally tensors with specific sparsity
  properties.  However, existing tensor processing systems require
  specialized extensions in order to take advantage of every new
  storage formats.  In this paper we describe a system that allows
  users to define flexible storage formats, using a declarative tensor
  query language, similar to the language used by the tensor program.
  The programmer only needs to write {\em storage mappings}, which
  describe, in a declarative way, how the tensors are laid out in main
  memory.  Then, we describe a \revb{cost-based optimizer} that optimizes the
  tensor program for the specific memory layout.  We demonstrate
  empirically significant performance improvements compared to
  state-of-the-art tensor processing systems.
\end{abstract}

